Solving mathematical programs with complementarity constraints arising in nonsmooth optimal control

This paper examines solution methods for mathematical programs with complementarity constraints (MPCC) obtained from the time-discretization of optimal control problems (OCPs) subject to nonsmooth dynamical systems. The MPCC theory and stationarity concepts are reviewed and summarized. The focus is on relaxation-based methods for MPCCs, which solve a (finite) sequence of more regular nonlinear programs (NLP), where a regularization/homotopy parameter is driven to zero. Such methods perform reasonably well on currently available benchmarks. However, these results do not always generalize to MPCCs obtained from nonsmooth OCPs. To provide a more complete picture, this paper introduces a novel benchmark collection of such problems, which we call nosbench. The problem set includes 603 different MPCCs and we split it into a few representative subsets to accelerate the testing. We compare different relaxation-based methods, NLP solvers, homotopy parameter update and relaxation parameter steering strategies. Moreover, we check whether the obtained stationary points allow first-order descent directions, which may be the case for some of the weaker MPCC stationarity concepts. In the best case, the Scholtes' relaxation [Scholtes, 2002] with IPOPT [W\"achter and Biegler, 2006] as NLP solver manages to solve 73.8 % of the problems. This highlights the need for further improvements in algorithms and software for MPCCs.

==> images/tabAccuracy.tex <==
\begin{table}[ht]
\centering
% spacing in table
\ra{1.3}
\begin{tabular}{@{}lr@{}}
  \toprule
  Type & Accuracy\\ \midrule
  A    & 82.47 $\pm$ 3.21 \\
  B    & 78.47 $\pm$ 2.43 \\
  C    & 84.30 $\pm$ 2.35 \\
  D    & 86.81 $\pm$ 3.01 \\
  \bottomrule
\end{tabular}

    \caption[Table caption]{\textbf{Table caption.} foo bar...\\}
    \label{tab:accuracy}
\end{table}
